Star algorithm for NN ensembling

Neural network ensembling is a common and robust way to increase model efficiency. In this paper, we propose a new neural network ensemble algorithm based on Audibert's empirical star algorithm. We provide optimal theoretical minimax bound on the excess squared risk. Additionally, we empirically study this algorithm on regression and classification tasks and compare it to most popular ensembling methods.

==> boston150f3.tex <==
\begin{table}[ht!]
\begin{tabular}{|l|lllllll|}
\hline
Name                    & d & MSE          & MAE   & MAPE  & $R^2$ & TRAIN MSE & TIME \\
\hline \hline
Snap Star (shot warm-up)   & 5 & 10.809±0.343 & 2.190 & 0.112 & 0.870     & 1.180      & 32.6 \\
Snap Star (new warm-up)    & 5 & 10.455±0.483 & 2.168 & 0.112 & 0.874     & 1.395     & 37.0 \\
Snap Star               & 5 & 10.400±0.586 & 2.150 & 0.110 & 0.875     & 1.359     & 39.6 \\
Snap Ensemble           & 5 & 11.045±0.496 & 2.216 & 0.115 & 0.867     & 1.630      & 39.4 \\
Ensemble                & 5 & 10.464±0.762 & 2.193 & 0.114 & 0.874     & 2.326     & 33.4 \\
Classic Star (new warm-up) & 5 & \textbf{9.756±0.328}  & 2.111 & 0.108 & 0.883     & 1.475     & 37.0 \\
Classic Star            & 5 & 10.415±0.648 & 2.153 & 0.110 & 0.875     & 1.605     & 40.2 \\
Big NN                 & 5 & 12.373±1.789 & 2.257 & 0.110 & 0.851     & 1.667     & 21.4 \\
\hline
Snap Star (shot warm-up)   & 4 & 10.600±0.911 & 2.168 & 0.112 & 0.873     & 1.204     & 27.2 \\
Snap Star (new warm-up)    & 4 & 10.251±0.873 & 2.150 & 0.109 & 0.877     & 1.543     & 31.2 \\
Snap Star               & 4 & 10.533±0.867 & 2.161 & 0.111 & 0.874     & 1.598     & 33.0 \\
Snap Ensemble           & 4 & 11.195±0.573 & 2.223 & 0.115 & 0.866     & 1.849     & 33.4 \\
Ensemble                & 4 & 11.186±0.315 & 2.228 & 0.115 & 0.866     & 2.168     & 27.2 \\
Classic Star (new warm-up) & 4 & \textbf{9.893±0.279}  & 2.135 & 0.108 & 0.881     & 1.428     & 30.2 \\
Classic Star            & 4 & 10.220±0.482 & 2.143 & 0.108 & 0.877     & 1.552     & 32.4 \\
Big NN                 & 4 & 12.114±2.446 & 2.299 & 0.113 & 0.855     & 2.109     & 18.2 \\
\hline
Snap Star (shot warm-up)   & 3 & 10.694±0.511 & 2.181 & 0.111 & 0.872     & 1.332     & 22.0 \\
Snap Star (new warm-up)    & 3 & 10.634±0.376 & 2.190 & 0.115 & 0.872     & 1.388     & 24.2 \\
Snap Star               & 3 & 11.705±0.866 & 2.235 & 0.114 & 0.859     & 1.596     & 26.2 \\
Snap Ensemble           & 3 & 10.916±0.459 & 2.198 & 0.113 & 0.869     & 1.742     & 25.8 \\
Ensemble                & 3 & 11.214±1.063 & 2.221 & 0.115 & 0.865     & 2.330      & 22.0 \\
Classic Star (new warm-up) & 3 & \textbf{9.585±0.658}  & 2.103 & 0.108 & 0.885     & 1.578     & 24.0 \\
Classic Star            & 3 & 9.781±0.456  & 2.121 & 0.109 & 0.883     & 1.567     & 26.0 \\
Big NN                 & 3 & 11.203±1.653 & 2.244 & 0.116 & 0.865     & 2.258     & 15.2 \\
\hline
Snap Star (shot warm-up)   & 2 & 11.414±0.390 & 2.243 & 0.115 & 0.863     & 1.534     & 16.4 \\
Snap Star (new warm-up)    & 2 & 11.541±1.366 & 2.267 & 0.115 & 0.861     & 2.004     & 19.0 \\
Snap Star               & 2 & 10.829±0.563 & 2.223 & 0.114 & 0.870     & 1.652     & 19.6 \\
Snap Ensemble           & 2 & 11.607±0.439 & 2.270 & 0.117 & 0.861     & 1.997     & 19.4 \\
Ensemble                & 2 & 11.579±1.636 & 2.255 & 0.115 & 0.861     & 2.650      & 16.2 \\
Classic Star (new warm-up) & 2 & \textbf{9.882±0.547}  & 2.117 & 0.109 & 0.881     & 1.637     & 18.2 \\
Classic Star            & 2 & 10.662±0.658 & 2.166 & 0.110 & 0.872     & 1.577     & 19.4 \\
Big NN                 & 2 & 11.471±1.203 & 2.288 & 0.118 & 0.862     & 2.011     & 12.0 \\
\hline
\end{tabular}
\caption{BOSTON HOUSE PRICING. Part of results at 150 epochs, $p=0.1$, $lr=0.01$}
\label{table:boston150}
\end{table}

==> boston75f3.tex <==
\begin{table}
\scalebox{1}{

\begin{tabular}{|l|lllllll|}
\hline
Name                    & d & MSE          & MAE   & MAPE  & $R^2$ & TRAIN MSE & TIME \\
\hline
\hline
Snap Star (shot warm-up)   & 5 & 10.811±0.973 & 2.202 & 0.111 & 0.870     & 1.499     & 18.0 \\
Snap Star (new warm-up)    & 5 & \textbf{9.948±0.930}  & 2.168 & 0.113 & 0.881     & 1.636     & 19.8 \\
Snap Star               & 5 & 11.065±0.852 & 2.218 & 0.114 & 0.867     & 1.688     & 20.8 \\
Snap Ensemble           & 5 & 11.143±0.747 & 2.236 & 0.116 & 0.866     & 1.932     & 21.2 \\
Ensemble                & 5 & 10.531±0.636 & 2.230 & 0.119 & 0.874     & 2.74      & 37.0 \\
Classic Star (new warm-up) & 5 & 10.533±0.582 & 2.169 & 0.112 & 0.874     & 2.094     & 19.8 \\
Classic Star            & 5 & 10.602±0.442 & 2.178 & 0.112 & 0.873     & 1.992     & 21.2 \\
Big NN                 & 5 & 11.791±2.704 & 2.289 & 0.116 & 0.858     & 2.708     & 11.6 \\
\hline
\end{tabular}
}
\caption{BOSTON HOUSE PRICING. Part of results at 75 epochs, $p=0.1$, $lr = 0.01$}
\label{table:boston75}
\end{table}

==> checklist.tex <==
\section*{Checklist}
\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Limitations are discussed in Section \ref{discussion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{This work is focused on the development of a new method of ensembling of neural networks.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Full set of assumptions of all theoretical results are discussed in the Section \ref{main_part}.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{We present all the proofs in Appendix \ref{Appendix A}.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We will submit our code as part of the supplemental material. After the review period, we plan to open-source the code, but not before in order to not break anonymity of the submission.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report the average value of the errors and their deviation in the Secction \ref{datasets}.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Resources for training models on each dataset are reported in the Section \ref{datasets}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Citations to the creators are provided in Section \ref{datasets}.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We did not curate/released new assets.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> cifar10.tex <==
    
\subsection{CIFAR-10}
    CIFAR-10 is image classification dataset consisting of 60000 $32 \times 32 \times 3$ colour images evenly distributed 10 classes. Dataset is divided to train and test in $5:1$ proportion.\\
    Small resnet-like convolutional neural network architecture was used in this experiment. This model starts with Convolution-MaxPool-BatchNorm layer combination repeated twice. Then, 4 residual blocks with ReLU - Convolution - BatchNorm are repeated. Then, output is flattened and two Linear layers with ReLU activations are applied to it.
    \begin{align*}
        x &= (Conv2d \circ MaxPool2d \circ BatchNorm2d \circ Conv2d \circ MaxPool2d \circ BatchNorm2d) (input)\\
        x_1 &= x + (ReLU \circ Conv2d \circ BatchNorm2d \circ  ReLU \circ Conv2d \circ BatchNorm2d) (x)\\
        x_2 &= x_1 + (ReLU \circ Conv2d \circ BatchNorm2d \circ  ReLU \circ Conv2d \circ BatchNorm2d) (x_1)\\
        x_3 &= (Conv2d \circ AvgPool2d)(x_2) +\\
            &+ (ReLU \circ Conv2d[stride=2] \circ BatchNorm2d \circ  ReLU \circ Conv2d \circ BatchNorm2d) (x_2)\\
        x_4 &= x_3 + (ReLU \circ Conv2d \circ BatchNorm2d \circ  ReLU \circ Conv2d \circ BatchNorm2d) (x_3)\\
        output &= (Linear \circ ReLU \circ Linear) (x_4.flatten())
    \end{align*}
    \textcolor{green}{Replace with resnet-18}\\
    \\
    The results are provided in table \ref{table:CIFAR10}.
    
    \begin{table}[ht!]
    \centering
    \begin{center}
    \begin{tabular}{ |c|c|c|c|c }
        \hline
        model type & number of models & test accuracy & entropy \\
        \hline
        base & 1 & $0.753 \pm 0.009$ & $0.734 \pm 0.016$ \\
        \hline
        ensemble & 2 & $0.788 \pm 0.009$ & $0.61 \pm 0.018$ \\
        & 3 & $0.804 \pm 0.006$ & $0.567 \pm 0.016$ \\
        & 4 & $0.81 \pm 0.007$ & $0.545 \pm 0.016$ \\
        & 5 & $0.813 \pm 0.008$ & $0.534 \pm 0.019$ \\
        & 6 & $0.815 \pm 0.007$ & $0.528 \pm 0.02$ \\
        \hline
        classic star & 2 & $0.778 \pm 0.001$ & $0.663 \pm 0.0$ \\
        & 3 & $0.797 \pm 0.005$ & $0.584 \pm 0.01$ \\
        & 4 & $0.807 \pm 0.004$ & $0.552 \pm 0.013$ \\
        & 5 & $0.814 \pm 0.004$ & $0.536 \pm 0.015$ \\
        & 6 & $0.816 \pm 0.006$ & $0.526 \pm 0.018$ \\
        \hline
        parallel & 2 & $0.776 \pm 0.004$ & $0.695 \pm 0.025$ \\
        & 3 & $0.789 \pm 0.002$ & $0.661 \pm 0.03$ \\
        & 4 & $0.8 \pm 0.004$ & $0.695 \pm 0.025$ \\
        & 5 & $0.796 \pm 0.002$ & $0.661 \pm 0.03$ \\
        & 6 & $0.796 \pm 0.004$ & $0.695 \pm 0.025$ \\
        \hline  
        snapshot base & 1 & $0.754 \pm 0.022$ & $0.718 \pm 0.054$ \\
        \hline
        SSE & 2 & $0.772 \pm 0.003$ & $0.664 \pm 0.008$ \\
        & 3 & $0.774 \pm 0.004$ & $0.655 \pm 0.008$ \\
        & 4 & $0.776 \pm 0.005$ & $0.656 \pm 0.008$ \\
        & 5 & $0.777 \pm 0.004$ & $0.657 \pm 0.008$ \\
        & 6 & $0.778 \pm 0.005$ & $0.658 \pm 0.008$ \\
        \hline
        snap star & 2 & $0.775 \pm 0.002$ & $0.67 \pm 0.008$ \\
        & 3 & $0.776 \pm 0.003$ & $0.669 \pm 0.01$ \\
        & 4 & $0.776 \pm 0.003$ & $0.669 \pm 0.009$ \\
        & 5 & $0.776 \pm 0.004$ & $0.669 \pm 0.009$ \\
        & 6 & $0.777 \pm 0.003$ & $0.668 \pm 0.009$ \\
        \hline
    \end{tabular}
    \end{center}
    \caption{Results on CIFAR-10 dataset}
    \label{table:CIFAR10}
    \end{table}


==> geom_ineq.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=1]{geom_ineq_picture.png}
    \caption{The cut surface $\mathcal{L}$}
    \label{fig:geom_ineq_picture}
\end{figure}    

    \begin{lemma}{(Geometric inequality for exact $Star_d$ estimator in the second step)}\\
    \label{geom_ineq_lemma-1}
    Let $\hat{g}_1 \ldots \hat{g}_d$ be  $\Delta_1$-empirical risk minimizers, $\wave{f}$ be the exact minimizer from the first and second step in $Star_d$ procedure respectively. Then for $c_{\ref{geom_ineq_lemma-1}}=\frac{1}{18}$ it satisfies:
    \begin{equation}
    \label{geom_ineq_ineq-1}
        \HE (h - Y)^2 - \HE (\wave{f} - Y)^2  \ge c_{\ref{geom_ineq_lemma-1}} \HE (\wave{f} - h)^2 - 2\Delta_1.
    \end{equation}
    \end{lemma}
\begin{proof}
    For any function $f,g$ we denote the empirical $\ell_2$ distance to be $\|f\|_n := \left[\HE f^2\right]^\frac{1}{2}$, empirical product to be $\langle f, g \rangle_n := \HE{[fg]}$ and the square of the empirical distance between $\mathcal{F}$ and $Y$ as
    $r_1$. %:= \min_{f \in \mathcal{F}}\|f - Y\|_n^2$ .
    By definition of $Star_d$ estimator for some $\lambda \in [0;1]$ we have:
    \begin{align*}
        \widehat{f} = (1 - \lambda) \widehat{g} + \lambda f
    \end{align*}    
    where $\widehat{g}$ lies in a convex hull of $\Delta$-empirical risk minimizers $\{\widehat{g}_i\}_{i=1}^d$.  %Since we are considering the case of inaccurate optimization, it will be useful to introduce a next value:
    %\begin{equation*}
    %    \Delta_1' := \max (\|\widehat{g}-Y\|^2_n - r_1 , 0) \leq %\Delta_1.
    %\end{equation*}
    Denote the some balls centered at $Y$ to be $\mathcal{B}_1 := \mathcal{B}(Y, \sqrt{r_1})$, $\mathcal{B}_1' := \mathcal{B}(Y, \|\widehat{g}-Y\|_n)$ and $\mathcal{B}_2 := \mathcal{B}(Y, \|\wave{f} - Y\|_n)$. The corresponding spheres will be called as $\mathcal{S}_1, \mathcal{S}_1', \mathcal{S}_2$. We have $\mathcal{B}_2 \subseteq \mathcal{B}_1$ and $\mathcal{B}_2 \subseteq \mathcal{B}_1'$. Denote by $\mathcal{C}$ the conic hull of $\mathcal{B}_2$ with origin $\widehat{g}$. Define the spherical cap outside the cone $\mathcal{C}$ to be $\mathcal{S} = \mathcal{S}'_1 \setminus \mathcal{C}$.
    
    First, $\wave{f} \in \mathcal{B}_2$ and it is a contact point of $\mathcal{C}$ and $\mathcal{S}_2$. Indeed, $\wave{f}$ is necessarily on a line segment between $\hat{g}$ and a point outside $\mathcal{B}_1$ that does not pass through the interior of $\mathcal{B}_2$ by optimality of $\wave{f}$. Let $K$ be the set of all contact points - potential locations of $\wave{f}$.
    
    Second, for any $h \in \mathcal{F}$, we have $\|h - Y\|_n \ge \sqrt{r_1}$ i.e. any $h \in \mathcal{F}$ is not in the interior of $\mathcal{B}_1$. Furthermore, let $\mathcal{C}'$ be finite cone with base at $K$ and apex $\hat{g}$ (so, $\mathcal{C}'$ is subset of cone $\mathcal{C}$ cut at $K$). Thus $h \in (int \mathcal{C})^c \cap (\mathcal{B}_1)^c$ or $h \in \mathcal{T}$, where $\mathcal{T} := \mathcal{C}' \cap \mathcal{B}_1^c$.

    Now we fix $h \in \mathcal{F}$ and consider the two dimensional plane $\mathcal{L}$ that passes through three points $(\hat{g}, Y, h)$, depicted in picture \ref{fig:geom_ineq_picture}. Observe that the left-hand-side of the desired inequality \ref{geom_ineq_ineq-1} is constant as $\wave{f}$ ranges over $K$. To prove the inequality it therefore suffices to choose a value $f' \in K$ that maximizes the right-hand-side. The maximization of $\|h - f'\|^2_n$ over $f' \in K$ is achieved by $f' \in K \cap \mathcal{L}$. This can be argued simply by symmetry: the two-dimensional plane $\mathcal{L}$ intersects $span(K)$ in a line and the distance between $h$ and $K$ is maximized at the extreme point of this intersection. Hence, to prove the desired inequality, we can restrict our attention to the plane $\mathcal{L}$ and $f'$ instead of $\wave{f}$.
    For any $h \in \mathcal{F}$, define the projection of $h$ onto the shell $L \cap S_1'$ to be $h_\perp$. By the geometry of the cone and triangle inequality we have:
    $$
        \|f' - \widehat{g}\|_n \ge \frac{1}{2}\|\widehat{g} - h_\perp\|_n \ge \frac{1}{2}\left(\|f' - h_\perp\|_n - \|f' - \widehat{g}\|_n\right),
    $$
    and, hence, $\|f' - \widehat{g}\|_n \geq \|f' - h_\perp\|_n / 3$.
    By the Pythagorean theorem,
    $$
        \|h_\perp - Y\|^2_n - \|f' - Y\|^2_n = \|\hat{g} - Y\|^2_n - \|f' - Y\|^2_n = \|f' - \hat{g}\|_n^2 \ge \frac{1}{9}\|f' - h_\perp\|^2_n.
    $$
    We can now extend this claim to $h$. Indeed, due to the fact that $h \in (int \mathcal{C})^c \cap (int\mathcal{B}_1)^c$ or $h \in \mathcal{T}$ and the geometry of the projection $h \to h_\perp$ there are 2 possibilities:
    
    a) $h \in (\mathcal{B}'_1)^c$. Then $\langle h_\perp - Y, h_\perp - h\rangle_n \le 0$.
    
    b) $h \in \mathcal{B}'_1$. Then, since $h \in (\mathcal{B}_1)^c$, we have
    $$
        \langle h_\perp - Y, h_\perp - h\rangle_n \leq \big(\|h-Y\|+\|h-h_\perp\|\big)\|h-h_\perp\| \le \|h_\perp - Y\|^2_n - \|h-Y\|^2_n \leq \Delta_1.
    $$
    In both cases, the following inequality is true
        \begin{align*}
            \|h - Y\|_n^2 - \|f' - Y\|_n^2
            &= \|h_\perp - h\|_n^2 - 2\langle h_\perp - Y, h_\perp - h\rangle_n + (\|h_\perp - Y\|_n^2 - \|f' - Y\|_n^2)\\
            &\ge \|h_\perp - h\|_n^2 - 2\Delta_1 + \frac{1}{9}\|f' - Y\|_n^2 \ge \frac{1}{18}\|f' - h\|_n^2 - 2\Delta_1.
        \end{align*}
\end{proof}

\begin{lemma}[Geometric Inequality for $\Delta$-empirical minimizers]
    \label{geom_ineq}
    Let $\hat{g}_1 \ldots \hat{g}_d$ be  $\Delta_1$-empirical risk minimizers, $\widehat{f}$ be the $\Delta_2$-empirical risk minimizer from the first and second step in $Star_d$ procedure respectively. Then for any $h \in \mathcal{F}$ and $c_{\ref{geom_ineq}} = \frac{1}{36}$ satisfies
    \begin{equation*}
        \widehat{\E} (h - Y)^2 - \widehat{\E}(\widehat{f} - Y)^2  \ge c_{\ref{geom_ineq}} \widehat{E}(\widehat{f} - h)^2 - 2(1+c_{\ref{geom_ineq}})[\Delta_1 +\Delta_2].
    \end{equation*}
\end{lemma}
\begin{proof}
    Since lemma \ref{geom_ineq_lemma-1} was actually proven for any $f \in K$, let $f''$ be the closest point to $\widehat{f}$ from $K$.      
    For this $f''$ holds \ref{geom_ineq_ineq-1}. Similarly to lemma \ref{geom_ineq_lemma-1}, there are 2 options: either $\widehat{f} \in (int\mathcal{C})^c$, or $\widehat{f} \in \mathcal{T}$.
    
    a) Let $\widehat{f} \in (int\mathcal{C})^c$, $\sqrt{\Delta_\parallel}$ and $\sqrt{\Delta_\perp}$ be lengths of parallel and perpendicular components of $\hat{f} - f''$ with respect to line $(\widehat{g}, f'')$.
    Since $\widehat{f}$ is $\Delta_2$-empirical risk minimizer, we have:
    $$
        \|\widehat{f} - f''\|^2 = \Delta_\perp + \Delta_\parallel
        \le \|\widehat{f} - Y\|_n^2 - \|f'' - Y\|_n^2 \leq \Delta_2.
    $$    
    
    b) Let $\widehat{f} \in \mathcal{T}$, then by the cosine theorem: $$
    \| \widehat{f} - f''\|^2_n = \|f''- Y \|^2_n + \| \widehat{f} - Y\|^2_n - 2 \|f''-Y\|_n \| \widehat{f}-Y\|_n \cos(\varphi').$$
    But $\cos(\varphi') \geq \cos(\varphi) = \frac{\|f''-Y\|_n}{\|\widehat{g}-Y \|_n}$ and $\|\widehat{f}-Y\|^2_n \geq r_1$.
    Then we have:
    \begin{align*}
        \|\widehat{f}-f''\|^2_n &\leq \Delta_2 + 2 \| f''- Y\|^2_n \left(1-\frac{\| \widehat{f}-Y\|_n}{\|\widehat{g}-Y \|_n}\right) \\
        &\leq \Delta_2 + 2\frac{ \| f''- Y\|^2_n}{\|\widehat{g}-Y \|_n}\left(\frac{\|\widehat{g}-Y \|^2_n -  \| \widehat{f}-Y\|^2_n}{\|\widehat{g}-Y \|_n+\| \widehat{f}-Y\|_n}\right) \leq \Delta_1 + \Delta_2.
    \end{align*}
    
    Lemma \ref{geom_ineq_lemma-1} states, that:
    $$
        \|h - Y\|_n^2 \ge \|f'' - Y\|_n^2 + c_{\ref{geom_ineq_lemma-1}} \|f'' - h\|_n^2 - 2\Delta_1.
    $$
    By using triangle inequality and convexity of a quadratic function
    we can get following bound
    \begin{align*}
        \frac{c_{\ref{geom_ineq_lemma-1}}}{2} \|\hat{f} - h\|^2_n  \le c_{\ref{geom_ineq_lemma-1}}\left(\|\hat{f} - f''\|_n^2 + \|f'' - h\|_n^2\right) \le  c_{\ref{geom_ineq_lemma-1}}[\Delta_2+\Delta_1]+ c_{\ref{geom_ineq_lemma-1}}\|f'' - h\|_n^2.
    \end{align*}
    Combining everything together and taking $c_{\ref{geom_ineq}}=\frac{c_{\ref{geom_ineq_lemma-1}}}{2}=\frac{1}{36}$, we get the required result
    $$
        \widehat{\E} (h - Y)^2 - \widehat{\E}(\hat{f} - Y)^2  \ge c_{\ref{geom_ineq}} \cdot \widehat{\E}(\hat{f} - h)^2 - 2(1+c_{\ref{geom_ineq}})[\Delta_1 + \Delta_2].
    $$
\end{proof}

==> old_files/experiments_old.tex <==
{\section{Experiments}
\label{experiments}}

\subsection{Description}
\begin{wrapfigure}{r}{0.6\textwidth}
\begin{algorithmic}[1]
\Procedure{Star}{$\mathcal{F},k$}
\State $r_1\gets calculate\_erm(set = \mathcal{F}, seed = seed_1)$
\State \dots
\State $r_k\gets calculate\_erm(set = \mathcal{F}, seed = seed_k)$
\State $\hat{f}^{s} \gets calculate\_erm(set = [r_1, \dots, r_k, \mathcal{F}], seed = seed)$
\State \textbf{return}  $\hat{f}^{s}$
\EndProcedure

\captionof{algorithm}{Modified star algorithm (correct for the finite $\mathcal{F}$)}
\end{algorithmic}
\end{wrapfigure}

As a class of functions $\mathcal{F}$, we will have many neural networks with a fixed architecture.
In the first step, we optimize the weights of k neural network models of a given architecture by training them independently of each other (black blocks on Fig \ref{starmod}).

\begin{wrapfigure}{r}{0.6\textwidth}
    \centering
        	\begin{tikzpicture}
    		\tikzstyle{unit}=[draw,shape=circle,inner sep=1pt,minimum size=0.5cm]
    		\tikzstyle{ridden}=[draw=red!,shape=rectangle,inner sep=1pt,minimum size=0.75cm]
    		\tikzstyle{hidden}=[draw, shape=rectangle,inner sep=1pt,minimum size=0.75cm]
     
    		\node[unit](x0) at (0,4.75){\small $x_1$};
    		\node[unit](x1) at (0,3.75){\small $x_2$};
    		\node at (0,3.125){\vdots};
    		\node[unit](xd) at (0,2.25){\small $x_d$};
     
    		\node[hidden](h10) at (3,5.5){ $r_1$};
    		\node[hidden](h11) at (3,4.25){ $r_2$};
    		\node[font=\Huge] at (3,3){\vdots};
    		\node[hidden](h1m) at (3,1.75){ $r_{k}$};
    		\node[hidden,red](h1m1) at (3,0.5){$f$};
     
    		\node[hidden, red](y) at (6,3.5){$\hat{f}^s$};
    		
     
    		\draw[->] (x0) -- (h10);
    		\draw[->] (x0) -- (h11);
    		\draw[->] (x0) -- (h1m);
    		\draw[->,red] (x0) -- (h1m1);
     
    		\draw[->] (x1) -- (h10);
    		\draw[->] (x1) -- (h11);
    		\draw[->] (x1) -- (h1m);
    		\draw[->,red] (x1) -- (h1m1);
    		
    		\draw[->] (xd) -- (h10);
    		\draw[->] (xd) -- (h11);
    		\draw[->] (xd) -- (h1m);
    		\draw[->,red] (xd) -- (h1m1);
    		
    		\draw[->, red] (h10) -- node [text width=2cm,midway,above right] {$\lambda_1$}(y);
    		\draw[->, red] (h11) -- node [text width=2cm,midway,below right] {$ $}(y);
    		\draw[->, red] (h1m) -- node [text width=2cm,midway,above] {$ $}(y);
    		\draw[->, red] (h1m1) -- node [text width=2cm,midway,below right] {$\lambda_{k+1}$}(y);
         	\end{tikzpicture}
    \captionof{figure}{Training scheme of the modified star algorithm}
    \label{starmod}
\end{wrapfigure}
Next, we add a new neural network and a connecting convex layer (red elements on Fig.\ref{starmod}).
Thus, by training a new model and weights for weighing at the second step, we simultaneously iterate over both the nodes of the simplices and the functions in them.

After we decide on the choice of the basic model, we will create two solutions (model Star and model nn, respectively). The first is the result of a two-step star algorithm. The second solution is the result of training a large neural network of a similar architecture using a standard method. In all cases, the Adam optimizer was used with lr = 0.01, $num\_model$ is the number of models that will be trained in the first step of the star algorithm (i.e. parameter k).

==> old_files/introduction_dima.tex <==
{\section{Dima/Introduction}
\label{introduction}}
    Deep neural networks is state-of-the-art machine learning algorithm in a wide variety of tasks; such as regression task or image classification. ImageNet image classification competition \cite{deng2009imagenet}, as well as many competitions in Kaggle \cite{kaggle} are dominated by deep learning models.\\
    \orange{\\Statistically, regression task may be formulated in the following way. Let  $S_n = \{(X_i,Y_i) : 1 \leq i \leq n\}$ be an sample of features-target independent pairs $(X_i,Y_i) \in \mathcal{X} \times {\mathcal{Y}}$ distributed according to some unknown distribution $\mathcal{P}$. Learning algorithm is a mapping $S_n \mapsto \hat{f}$, where $\widehat{f} \in \mathcal{G}$ ~-- class of neural networks with fixed architecture \textcolor{green}{and under some restrictions}. For regression task with MSE loss quality of an estimator $\hat{f}$ is measured with following risk:
    \begin{equation}
    \label{R'}
        R(\hat{f})=\E_{(X, Y) \sim \mathcal{P}}\big[(\hat{f}(X) - Y)^2\big].
    \end{equation}
    Here the expectation is taken with respect to a test pair $(X, Y)$, which is independent of the training sample $S_n$. (S: this is a description of the problem, not an introduction)}\\
    \\
    The most common way of training model is empirical risk minimization (ERM) on $\mathcal{G}$ via gradient methods. Empirical risk is defined as:
    \begin{equation}
    \label{r'}
        r(\hat{f}) = \frac{1}{n}\sum_{i=1}^n \big(\hat{f}(X_i) - Y_i\big)^2
    \end{equation}
    State-of-the-art result of \cite{schmidt2020nonparametric} provides following oracle inequality for neural networks:
    \begin{gather}
        R(\hat{f}) \le (1 + \varepsilon)^2\left(\inf_{f \in \mathcal{F}} \|f - \E(Y|X)\|_\infty^2 + \Delta_{\mathcal{F}}(\hat{f}) \right) + \frac{C\big(\varepsilon, \mathrm{Comp}(\mathcal{F})\big)\log n}{n},\\
        \text{where}\quad \Delta_{\mathcal{F}}(\hat{f}) = r(\hat{f}) - \underset{g \in \mathcal{F}}{\inf} r(g)
    \end{gather}
    Here $\mathrm{Comp}(\mathcal{F})$ depends on complexity of class $\mathcal{F}$. Notice, that inequality is not sharp because of the $(1 + \varepsilon)^2$ multiplier.\\
    \\
    It is well known, that classes of neural network functions are extremely non-convex, and ERM may not have the optimal rate of excess loss convergence for non-convex $\mathcal{G}$ \cite{lecue2009aggregation}. However, learning algorithm does not necessary has to output function from class $\mathcal{G}$. It's sufficient that $\mathcal{G}$ is chosen well, so that infimum risk of $\mathcal{G}$ is low; and that learning algorithm returns such function $f \in \mathcal{F}$, that its risk is close to that infimum. There are several thing to consider for optimal $\mathcal{F}$:
    \\
    \begin{itemize}
        \item Choosing $\mathcal{F}$ simply as another class of neural networks (with different architecture) does not solve non-convexity problem. We are rather motivated to look for meta-algorithm over neural networks in $\mathcal{G}$.
        \item Although the non-convexity is a cause of inoptimal convergence, \cite[Theorem A]{lecue2009aggregation} shows that convex hull $\mathrm{Conv}(\mathcal{G})$ also does not converge with fast rates. This function class is excessively wide, which leads to model overfitting.
        \item Approximation-estimation tradeoff states, that we wish to optimize $\hat{f}$ over function class rich enough to minimize approximation error; but not too wide to overfit, so estimation error is not excessively large.
        \item The prime example of such wider function class $\mathcal{F}$ is an ensemble of neural networks. Currently, best test results on most competitive datasets belong to ensembles as they are robust and effective meta-algorithms. This motivates us to search for ensemble-like meta-algorithm.
        \item On practice global loss minima are almost never reached for neural networks, as algorithm converges to local minima or saddle points. Therefore, it is important to consider approximate empirical risk minimizers in our analysis.
    \end{itemize}
    Our contribution is the following.
    \begin{itemize}
        \item We propose a multi-step empirical star aggregation algorithm based on empirical star algorithm by Audibert \cite{a07-mixture}.
        \item  We prove that the produced estimator satisfies a sharp oracle inequality with (almost) the same additional term as in the paper of Schmidt-Hieber and provide an upper bound on the generalization error for the case of approximate empirical risk minimizers. 
        \item We illustrate the performance of the proposed procedure empirically on regression and classification tasks, and compare it to ensemble of model average and convex combination of several models trained concurrently. \textcolor{green}{Maybe add a little more experiment info?}
    \end{itemize}
    The proposed algorithm is performed in several steps:
    \begin{itemize}
        \item First, $d$ approximate empirical risk minimizers from the base class are trained independently.
        \item After that, parameters of these models are fixed and another, non-trained model is added to them. Final model is composed of all $d+1$ models, connected by a linear layer with convex coefficients. The final layer and non-trained model are trained simultaneously.
    \end{itemize}
    On one hand proposed algorithm is similar to the model averaging, and on the other the optimizing function lies in the class between class of reference predictors $\mathcal{G}$ and its convex set.
    \orange{(S:How is our algorithm similar to averaging? and why is it important that the function lies somewhere between the convex hull and the original class?)}


==> old_files/introduction_old.tex <==
{\section{Introduction}
\label{introduction}}
    Deep neural networks is state-of-the-art machine learning algorithm in a wide variety of tasks. Most common of those tasks are regression and classification problems, image classification, speech recognition and others \red{(You need to insert some references to support this claim)}. Those problems may be formulated in the following way.\\
    \\
    Let  $S_n = \{(X_i,Y_i) : 1 \leq i \leq n\}$ be an sample of features-target independent pairs $(X_i,Y_i) \in \mathcal{X}\times{\mathcal{Y}}$ distributed according to some unknown distribution $\mathcal{P}$. A function mapping $\mathcal{X}$
    to $\mathcal{Y}$ is called a \textit{predictor}. A \textit{statistical estimator} is a procedure mapping the observed random 
    sample $S_n$ to some predictor $\hat{f} = \hat{f}(S_n)$. Quality of an estimator is measured by risk function. Risk for regression task with MSE loss is defined as:
    \begin{equation}
    \label{R'}
        R(\hat{f})=\E_{(X, Y) \sim \mathcal{P}}\big[(\hat{f}(X) - Y)^2\big].
    \end{equation}
    \red{N.P. The expectation is taken with respect to a test pair $(X, Y)$, which is independent of the training sample $S_n$.}\\
    The above performance measure is absolute, and its scale depends on the properties of the loss function $\ell$ as well as the distribution $\mathcal{P}$. In order to obtain a performance measure whose value can approach zero as the sample size $n$ increases, a class of \textit{reference predictors} $\mathcal{G}$ is introduced. The risk incurred by the estimator $\hat{f}$, relative to the smallest risk achievable via predictors in class $\mathcal{G}$, is called \textit{excess risk} and it is defined as
    \begin{equation}
    \label{excess_loss}
    \mathcal{E}_{\mathcal{G}}(\hat{f}) = R(\hat{f}) - \underset{g \in \mathcal{G}}{\inf} R(g),
    \end{equation}
    Optimal rate of convergence for $\mathcal{E}$ for finite class is well known \cite{optimal_rates}:
    $$
        \mathcal{E}_{\mathcal{G}}(\hat{f}) \sim \frac{|\mathcal{G}|}{n}
    $$
    For non-finite class corresponding rate is:
    $$
        \mathcal{E}_{\mathcal{G}}(\hat{f}) \sim C_\varepsilon\frac{1}{n} + O(\varepsilon)
    $$
    \\
    Notice, that training algorithm does not necessary has to output function from class $\mathcal{G}$. It's sufficient that $\mathcal{G}$ is chosen well, so that infimum risk of $\mathcal{G}$ is low; and that training algorithm returns such function $f \in \mathcal{F}$, that its excess risk w.r.t. $\mathcal{G}$ is small.\\
    \\
    The most common way of training model is empirical risk minimization (ERM) on $\mathcal{G}$ via gradient methods. Empirical risk is defined as:
    \begin{equation}
    \label{r'}
        r(\hat{f}) = \frac{1}{n}\sum_{i=1}^n \ell\big(\hat{f}(X_i), Y_i\big)
    \end{equation}
    Similarly we have excess empirical risk:
    \begin{equation}
    \label{emp_excess_loss}
    \Delta_{\mathcal{G}}(\hat{f}) = r(\hat{f}) - \underset{g \in \mathcal{G}}{\inf} r(g),
    \end{equation}
    State-of-the-art result of \cite{Schmidt-Hieber_2020} provides following oracle inequality for neural networks:
    $$
        R(\hat{f}) \le (1 + \varepsilon)^2\left(\inf_{f \in \mathcal{F}} \|f - \E(Y|X)\|_\infty^2 + \Delta_{\mathcal{F}}(\hat{f}) \right) + \frac{C(\varepsilon)\log n}{n}
    $$
    The inequality is not sharp because of the $(1 + \varepsilon)^2$ multiplier.\\
    \\
    It is well known, that classes of neural network functions are non-convex. Moreover, on practice global loss minima are almost never reached, as algorithm converges to local minima or saddle points; as architectures with overabundance of parameters are used. However, ERM may not have the optimal rate of excess loss convergence for non-convex $\mathcal{G}$ as well as for its convex hull $\mathrm{Conv}(\mathcal{G})$ \cite[Theorem A]{lecue2009aggregation}. Approximation-estimation tradeoff states, that we wish to optimize $\hat{f}$ over function class rich enough to minimize approximation error; but not too wide to overfit, so estimation error is not excessively large.\\
    \\
    Currently, best test results on most competitive datasets belong to neural network ensembles. One of the most widespread ensemble methods is model averaging. Averaging model outputs does not change bias, but (under assumption, that models are trained on independent sample sets) proportionally reduces variance, lowering overfitting effect.
    \\
    \red{N.P. Our contribution is the following.
    \begin{itemize}
        \item We propose a multi-step empirical star aggregation algorithm...
        \item We prove that...
        \item We illustrate the performance of the proposed procedure...
    \end{itemize}}
    We propose multi-step empirical star aggregation algorithm abased on empirical star algorithm by Audibert \cite{a07-mixture}. We prove that the produced estimator satisfies a sharp oracle inequality with (almost) the same additional term as in the paper of Schmidt-Hieber and provide an upper bound on the generalization error for the case of approximate empirical risk minimizers. On one hand proposed algorithm is similar to the model averaging, and on the other the optimizing function lies in the class between class of reference predictors $\mathcal{G}$ and its convex set.
{\section{Related work}
\label{related work}}
    \subsection{Ensembling methods}
    Neural network ensembles are popular due to their improved generalization and robustness, compared to single models. State-of-the-art deep learning ensembles are presented in review \cite{ensemble_review}.\\
    \\
    Other than explicit ensembles such as model averaging; implicit ensembling technique \textit{DropOut} is widely used (creating a de-facto ensemble from just one model by randomly zeroing neurons) \cite{dropout}.\\
    \\
    Main drawback of neural networks ensembles is high computational cost. Several neural networks ensembling methods aimed at reducing computational expenses were proposed in the recent years.
    \begin{itemize}
        \item \textit{Snapshot Ensembling} \cite{snapshots} trains one model with cyclic learning rate, reaching several loss minima, and saved model weights at those minima to ensemble them.
        \item \textit{Fast Geometric Ensembling} \cite{FGE} trains
    \end{itemize}
    \subsection{Star algorithm}
    Empirical star algorithm was firstly \red{(N. P. Use the words ``first'', ``second'', instead of ``firstly'', ``secondly'', etc.)} introduced for finite function classes by Audibert in \cite{a07-mixture}; it was proved to be optimal in expectation and deviation convergence rates.\\
    \\
    Our analysis is based on paper \cite{liang2015learning}, which shows optimality of star algorithm for wide variety of function classes with offset Rademacher complexity technique.\\
    This result is generalized in \cite{vijaykumar2021localization} for loss functions other than MSE, including exp-concave functions such as logistic loss.\\

==> old_files/oldintroduction.tex <==
{\section{Introduction}
\label{introduction}}


\textbf{General view of aggregation tasks}

Let  $S_n = (X_i,Y_i)^{n}_{i=1}$ i.i.d. sample of input-output pairs $(X_i,Y_i) \in \mathcal{X}\times{\mathcal{Y}}$ distributed according to some unknown distribution $\mathcal{P}$. A function mapping $\mathcal{X}$
to $\mathcal{Y}$ is called a \textit{predictor}. A \textit{statistical estimator} is a procedure mapping the observed random 
sample $S_n$ to some predictor $\hat{f} = \hat{f}(S_n)$. In order to measure the quality of an estimator $\hat{f}$, we introduce a loss function $\ell : \mathcal{Y} \times \mathcal{Y} \rightarrow [0, \infty)$ and define the performance measure called risk as follows:

\begin{equation}
\label{R'}
    R(\hat{f})=\mathbb{E}_{(X, Y) \sim \mathcal{P}}[\ell(\hat{f}(X),Y|S_n].
\end{equation}

The above performance measure is absolute, and its scale depends on the properties of the loss function $\ell$ as well as the distribution $\mathcal{P}$. In order to obtain a performance measure whose value
can approach zero as the sample size $n$ increases, it is customary to introduce a class of \textit{reference predictors} $\mathcal{G}$. The risk incurred by the estimator $\hat{f}$, relative to the smallest risk achievable via predictors in class $\mathcal{G}$, is called \textit{excess risk} and it is defined as


\begin{equation}
\label{excess_loss}
\mathcal{E}(\hat{f}) = R(\hat{f}) - \underset{g \in \mathcal{G}}{inf} R(g),
\end{equation}

Upper bounds on the excess risk $\mathcal{E} (\hat{f}, \mathcal{G})$ can be obtained either in \textit{expectation} or in \textit{deviation}. The former type of bounds aims to find the smallest remainder term $\Delta_{E}(n,\mathcal{G})$ that depends on properties of the estimator $\hat{f}$ such as its range $\mathcal{F}$ so that for some universal constant c > 0 the following holds:

\begin{equation}
\label{exp_loss}
\mathcal{E}_{S_n}[ R(\hat{f}) - \underset{g \in \mathcal{G}}{inf} R(g)] \leq c \Delta_{E}(n,\mathcal{G}).
\end{equation}



Similarly, bounds in deviation aim to find the smallest remainder term $\Delta_{Pr}$ that depends on properties of the estimator $\hat{f}$ so that the following holds for any $\delta \in (0, 1]$:

\begin{equation}
\mathbb{P}[ R(\hat{f}) - \underset{g \in \mathcal{G}}{inf} R(g) > c \Delta_{Pr}(n,\mathcal{G},\delta)] \leq \delta.
\end{equation}

Choosing in various ways $\mathcal{G}$ we will get different tasks aggregation. Let us have some finite class of predictors $\mathcal{F} = \{f_i\}^{M}_{i=1}$. In the case $\mathcal{G} = \mathcal{F}$ we get a \textit{model selection problem}, in the same cases $\mathcal{G} = Conv(\mathcal{F})$ and $\mathcal{G} = Lin(\mathcal{F})$ we get a  \textit{convex} and \textit{linear} aggregation problem respectively. These tasks were formulated in \cite{jn}. 


Aggregation under different losses was extensively studied in the literature.
The mean squared error was studied in \cite{jn}, \cite{yang04} and \cite{t03}.
Oracle inequalities for the $\varphi$-risk and, in particular, the hinge-risk were obtained 
in \cite{l07}, \cite{juditsky05} and \cite{jrt08}. In \cite{lm09}, optimal bounds in deviation for model selection with a loss function of the form $\ell(f, g) = \varphi(f - g)$ were derived. Model selection under $L_p$-risk was considered in \cite{g09}. Finally, aggregation under the Kullback-Leibler loss was studied in \cite{rig12} and \cite{b16}.


\textbf{Why is the aggregation problem interesting?(for nn may be)}

Model selection and aggregation procedures attract a lot of interest in statistics and machine learning. A good aggregation procedure can significantly empower performance of a bunch of weak learners or estimates.
Aggregation procedures have a wide range of applications and can be used in regression problems (\cite{t03}, \cite{yang04}), density estimation (\cite{ps06}, \cite{rt07}, \cite{l06}, \cite{ds17}) and classification problems (\cite{t04}, \cite{juditsky05}, \cite{ps06}).

In this paper, the aggregation procedure of neural networks is mainly studied. Aggregation of multiple neural networks by majority voting or averaging was studied in \cite{caruana2004ensemble}. It is known that combining the results of several deep models can reduce the number of errors. In fact, most high-profile contests, such as Imagenet \cite{deng2009imagenet} are won by ensembles of deep learning architectures.



\textbf{Why is it important to get estimates in deviations?}

The efficiency of an algorithm can be summarized by its expected risk, but this does not precise the fluctuations of its risk. In several application fields of learning algorithms, these fluctuations play a key role: in finance for instance, the bigger the losses can be, the more money the bank needs to freeze in order to alleviate these possible losses. In this case, a “good” algorithm is an algorithm having not only low expected risk but also small deviations.

\textbf{Known results for the problem model selection}


In \cite{lecue2009aggregation} the model selection problem was considered when labels and predictors are bounded by some constant $b$.
In this case for excess risk, the concept of the optimal order of convergence (in the sense of deviations) was formulated:
\begin{definition}
A function $\Delta(n, M )$ is an optimal rate of aggregation with confidence $0 < \delta < 1/2$ and a procedure $\tilde f$  is an optimal aggregation procedure with confidence $\delta$ if there exists a constant $c_1(\delta)$ for which the following hold:
\begin{enumerate}
    \item For any integers n and M, any set $\mathcal{F}$ of cardinality $M$ and any target $\mathcal{Y}$ (all bounded by $b$), with probability at least 1 - $\delta$, $\tilde f$ satisfies :
    $$R(\tilde f) - \underset{f \in \mathcal{F}}{min} R(f) \leq c_1(\delta)\Delta_{n,M}.
    $$
    \item
    There exists an absolute constant $c' > 0$ such that the following holds. For any  integers $M$ and $n$, and any procedure $\bar{f}$, there exist a set $\mathcal{F}$ of cardinality $M$ and a target $\mathcal{Y}$ (all bounded by $b$) such that, with probability at least $1/2$,
    $$R(\bar{f}) - \underset{f \in \mathcal{F}}{min} R(f) \geq c'\Delta_{n,M}.
    $$
\end{enumerate}
\end{definition}
In the same paper, it was proved that the optimal order for the model selection problem is 
\begin{equation}
\label{delta_ms}
\Delta^{MS}_{n,M} = \frac{\log M}{n}.
\end{equation}

This means that there is no aggregation algorithm for which it would be possible to guarantee uniformly over all possible finite classes $\mathcal{F}$ of functions bounded by some constant $b$ a better aggregation rate than $\frac{log(|\mathcal{F}|)}{n}$.

\begin{remark}
For the MSA problem, the order \eqref{delta_ms} is optimal both in terms of risk expectation \cite{t03} and in terms of deviations \cite{lecue2009aggregation}.
\end{remark}


The restoration of regression dependence can be considered as a natural development of the theory
of learning pattern recognition, which was studied by V.N.Vapnik. His monograph [Vap79] offers
a solution to the regression problem by minimizing empirical risk.

The MSA task is a special case of regression dependence recovery. It is known for her that if the aggregation algorithm is allowed to select a function from the original class $\mathcal{F}$, then the optimal
order of convergence of the algorithm errors will be $ \Delta_{n,M} = O\big(\sqrt{\frac{M}{n}}\big)$ \cite{lecue2009aggregation}.
The method of V.N.Vapnik applied to the original class of predictors just achieves this estimate.

To get closer to the speed \eqref{delta_ms}, it is necessary to expand the class of functions available for the algorithm.

Since optimal aggregation procedures representing a
convex combination of functions are known for some problems \cite{juditsky2008learning}, the idea naturally arises to minimize
empirical risk on a convex hull of class $\mathcal{F}$.

In the article \cite{lecue2009aggregation} this case was investigated and the following result was obtained: minimizing empirical risk
on a convex hull of class $\mathcal{F}$ does not give an optimal aggregation rate for the MSA problem. It also proposed an algorithm that achieves this estimate. At one of its stages, it is required to minimize the empirical risk on the convex hull of some random subclass, which complicates the practical implementation. Moreover, during the minimization of empirical risk, only a part of the sample can be used, which is a significant disadvantage with small amounts of data.

An alternative to this method is the star algorithm proposed by Audibert \cite{a07-mixture}. It minimizes the empirical risk for some intermediate between the original class and its convex hull of the set. This method has an optimal aggregation rate, does not impose restrictions on the joint distribution of $\mathcal{P}$. Its advantages are also the absence of hyperparameters and ease of implementation.

\textbf{How is the learning process related to model selection problem?}

Let's consider a situation when we solve some problem, for example, using a class of neural networks of fixed architecture $\mathcal{F}$. In fact, we want to choose from the $\mathcal{F}$ with the best generalizing ability, the quality criterion of which can be a real risk. That is, we minimize the excess risk.

Naturally, there is a desire to set a generalized model selection problem by removing the finiteness condition of the class $\mathcal{F}$. From the analysis of the finite case, we already know that the usual minimization
of empirical risk may not work well (in the case of non-convexity of class $\mathcal{F}$), so we propose to apply algorithms for solving model selection problem with optimal orders in the final case to train models.

\textbf{Generalized MSA}

We have an  $S_n = (X_i,Y_i)^{n}_{i=1}$ i.i.d. sample of input-output pairs $(X_i,Y_i) \in \mathcal{X}\times{\mathcal{Y}}$ distributed according to some unknown distribution $\mathcal{P}$. We also chose a certain family of solutions $\mathcal{F}$ (for example, a family of neural networks of a fixed architecture, but with different weights).
It is necessary to build an algorithm $\mathcal{A}$ that, based on a given sample $S_n$ and a class of predictors $\mathcal{F}$ (not necessarily finite), will build a new predictor $\hat{f}$ that minimizes excess risk:
$$
\mathcal{E}(\hat{f}) = R(\hat{f}) - \underset{f \in \mathcal{F}}{inf} R(f) \rightarrow min.
$$

In the classical msa problem, the optimal orders depend on the parameter $M = |\mathcal{F}|$. In the case of a generalized problem, we suggest using the parameter $\mathcal{N}$ - the number of nodes in $1/n$-net of class functions $\mathcal{F}$. Note that for sufficiently large $n$ for any finite class $|\mathcal{F}| = \mathcal{N}$. This allows us to assert that
the optimal order of the generalized problem (\textbf{ in a bounded case}) is bounded from below by  $\frac{\log \mathcal{N}}{n}$.

\textbf{ В идеале надо будет отказаться от ограниченности и показать выполнимость для нейронных сетей lower isometry bound}

{\section{Related Work}}
Наши результаты и использованные техники, потенциальные обобщения.

Offest Rademacher complexity (почему это круто) и exp-tail+др. (потенциальное обобщение на другие риски и другие типы задач :классификация, glm ... )


На практике в качестве $\mathcal{F}$ мы рассматриваем класс нейронных сетей с какой-то фиксированной архитектурой.  Мы предлагаем модификацию классического star-алгоритма (которая навеяна результатами экспериментов), обобщаем технику Рахлина и Лианга с offset Rademacher complexity \cite{liang2015learning} и показываем, что при выполнении некоторых условий (\textbf{Каких? Чтобы можно было оценкой снизу  для конечного случая воспользоваться}) предложенный алгоритм обладает скоростью сходимости порядка $O(\frac{\log n\cdot\mathcal{N}}{n})$, то есть является \textbf{оптимальным или оптимальным с точностью до логарифма}. 

Также в работе уделяется внимание устойчивости алгоритма: исследуется ситуация, когда поиск эмпирических минимизаторов на каждом шаге выполняется с некоторой погрешностью $\Delta$ и показывается, что избыточный риск в таком случае меняется $\sim$ на $\Delta$.


\textbf{offset Rademacher complexity} 

При анализе star-алгоритма основным моментом являлась ограниченность всех функций и применимость неравенства концентрации Бернштейна. В работе \cite{liang2015learning} пытаются отойти от этого условия, вводя ограничение lower isometry bound, но освобождаясь от требования ограниченности. Авторы одни из первых вводят понятие offset Rademacher complexity для анализа эмпирических минимизаторов. И показывают, что избыточный риск результата двухшагового алгоритма Одибера может быть ограничен сверху этой величиной (и в смысле отклонений, и в смысле ожиданий).

\textbf{exp-tail}

В работе \cite{kanade2022exponential} эта теория получает  продолжение.
Надо рассказать про связь с  классической теорией и важность этого направления.
Почему это удобно и почему это лучше.


\textbf{Применимость star-алгоритма с другими функциями ошибками и для других задач (\cite{kanade2022exponential})}

Но star-алгоритм применим не только для минимизации квадратичного риска. В работе \cite{vijaykumar2021localization} вводится обобщение свойства выпуклости ($\mu-d$ выпуклость) для функций и показывается, что для такого класса функций потерь механизм получения верхней оценки избыточного риска star-алгоритма через offset Rademacher complexity может быть также применен.
\textbf{Примеры задач, которые покрываются этим анализом и их важность (GLM,crossentropy)}


\textbf{Потенциально можно ускорить алгоритм техникой snapshot ensemble и его модификацией}

\textbf{Про то, то число локальных минимумов в нейросети растет экспоненциально с ростом параметров (\cite{kawaguchi2016deep})
Про важность различных моделей во время агрегации (\cite{caruana2004ensemble} \cite{deng2009imagenet}).}
 
 Это надо где-то в экспериментах.

==> old_files/trash.tex <==
The first lemma describes the behavior of offset Rademacher process for a finite class.
\begin{lemma}[Lemma 9 in \cite{liang2015learning}]
    Let $V \subseteq \mathbb{R}^n$ be finite set, $|V| = N$. Then for any $C > 0$:
    $$
        \mathbb{E}_{\sigma}\max_{v \in V}\left[\frac{1}{n}\sum_{i=1}^n\sigma_i v_i - Cv_i^2\right] \le M\frac{\log N}{n};
    $$
    for any $\delta > 0$
    $$
        {\Prob}_{\sigma}\left(\max_{v \in V}\left[\frac{1}{n}\sum_{i=1}^n\sigma_i v_i - Cv_i^2\right] > M\frac{\log N + \log \frac{1}{\delta}}{n}\right) \le \delta,
    $$
    where
    $$
        M := \sup_{v \in V \setminus \{0\}} \frac{\sum_{i =1}^n v_i^2 \xi_i^2}{2C\sum_{i =1}^n v_i^2}
    $$
\end{lemma}



    % First Th about excess loss expectation
    %\begin{theorem}
    %\textbf{Need to change it. Add info about fcnn.}
    %\label{th-4}
    %    The following expectation bound on excess loss of the $Star_d$ estimator holds:
        $$
    %        \E \mathcal{E}(\hat{f}) \le (2M + K(2+c)/2) \cdot \E \sup_{h \in \mathcal{H}} \left\{\frac{1}{n}\sum_{i=1}^{n} 2\sigma_i h(X_i) - c'h(X_i)^2\right\} + 2(1+c)[\Delta_1 + \Delta_2]
        $$
    %    where $\sigma_1, \ldots \sigma_n$ are independent Rademacher random variables, $c' = \min\left\{\frac{c}{4M}, \frac{c}{4K(2+c)}\right\}$, $K = \sup_{f \in \mathcal{F}} |f|_\infty$ and $M = \sup_\mathcal{F} |Y - f|_\infty$ almost surely.
    %\end{theorem}
    %[Text from \cite{liang2015learning}] While Theorem \ref{th-4} only applies to bounded functions and bounded noise, the upper bound already captures the localization phenomenon, even for non-convex function classes (and thus goes well beyond the classical local Rademacher analysis).
    %We need a  stronger assumption that will allow us to take this constant to be at least $1-\frac{c}{4}$. We phrase this condition—the lower isometry bound—as follows.

==> oldboston200.tex <==
\begin{table}[ht!]
\centering
\begin{tabular}{|l|lllllll|}
\hline
Name                    & d & MSE          & MAE   & MAPE  & $R^2$ & TRAIN MSE & TIME \\
\hline \hline
Snap Star (shot warm-up)   & 5 & 11.155±0.967 & 2.185 & 0.110 & 0.866     & 1.232     & 52.4 \\
Snap Star (new warm-up)    & 5 & 10.677±1.034 & 2.148 & 0.110 & 0.872     & 1.306     & 49.2 \\
Snap Ensemble           & 5 & 11.123±0.615 & 2.206 & 0.114 & 0.866     & 1.728     & 43.4 \\
Ensemble                & 5 & 10.172±0.621 & 2.164 & 0.113 & 0.878     & 2.133     & 43.2 \\
Classic Star (no warm-up)  & 5 & \textbf{9.650±0.911}  & 2.092 & 0.108 & \textbf{0.884}     & 1.373     & 52.0 \\
Classic Star (new warm-up) & 5 & 9.664±0.324  & \textbf{2.086} & \textbf{0.107} & \textbf{0.884}     & 1.374     & 45.8 \\
Big NN                  & 5 & 12.117±1.601 & 2.326 & 0.115 & 0.854     & 2.160     & 28.4 \\
\hline
Snap Star (shot warm-up)   & 4 & 10.745±0.640 & 2.154 & 0.109 & 0.871     & 1.192     & 43.0 \\
Snap Star (new warm-up)    & 4 & 10.862±0.537 & 2.162 & 0.109 & 0.870     & 1.401     & 43.0 \\
Snap Ensemble           & 4 & 11.169±0.558 & 2.205 & 0.113 & 0.866     & 1.679     & 36.0 \\
Ensemble                & 4 & 9.967±0.244  & 2.144 & 0.112 & 0.880     & 1.833     & 35.8 \\
Classic Star (no warm-up)  & 4 & 9.887±0.501  & \textbf{2.111} & \textbf{0.108} & 0.881     & 1.326     & 43.6 \\
Classic Star (new warm-up) & 4 & \textbf{9.741±0.790}  & 2.114 & 0.109 & \textbf{0.883}     & 1.400     & 38.2 \\
Big NN                  & 4 & 11.856±0.429 & 2.323 & 0.118 & 0.858     & 1.937     & 24.0 \\
\hline
Snap Star (shot warm-up)   & 3 & 10.255±0.582 & 2.158 & 0.110 & 0.877     & 1.280     & 35.0 \\
Snap Star (new warm-up)    & 3 & 9.947±0.434  & 2.135 & 0.110 & \textbf{0.881}     & 1.336     & 32.8 \\
Snap Ensemble           & 3 & 10.858±0.533 & 2.211 & 0.114 & 0.870     & 1.773     & 29.0 \\
Ensemble                & 3 & \textbf{9.941±0.627}  & 2.175 & 0.115 & \textbf{0.881}     & 2.009     & 28.8 \\
Classic Star (no warm-up)  & 3 & 10.138±0.605 & \textbf{2.128} & \textbf{0.108} & 0.878     & 1.500     & 34.2 \\
Classic Star (new warm-up) & 3 & 10.255±0.742 & 2.140 & \textbf{0.108} & 0.877     & 1.644     & 29.2 \\
Big NN & 3 & 10.714±1.044 & 2.203 & 0.113 & 0.871     & 1.215     & 19.4 \\
\hline
\end{tabular}
\caption{BOSTON HOUSE PRICING. Part of results at 200 epochs, $p=0.1$, $lr=0.01$}
\label{table:boston200}
\end{table}

==> setting-up.tex <==
\subsection{Setting up}
    The first $d$ models are produced exactly as in classical (model averaging) ensembles: $d$ neural networks are randomly initialized and trained independently for chosen number of epoches. We used \orange{Adam optimizer in the experiments below; base models were chosen depending on the task. Despite the fact, that our theoretical analysis provides proof of optimal convergence rate only for MSE loss function; generalization for exp-concave losses are possible, as shown in \cite{vijaykumar2021localization}. This motivates us to also examine performance of star algorithm on the image classification tasks also.\\
    \\
    Convexity of last layer coefficients in the last step of algorithm plays important role in theoretical analysis. To ensure convexity, softmax of weights $w_1 \ldots w_{d+1} \in \mathbb{R}$ is taken prior to multiplication with outputs of all $d+1$ models.\\}
    As with classical model averaging ensembles, star algorithm suffers from high computational expenses. To combat this drawback, we used snapshot ensembling \cite{snapshots} technique. This allows us to train models for star algorithm with budget equivalent to single model training.\\
    In theory, the last model is simply optimized over chosen neural network function class simultaneously with last layer. In practice, however, initialization of the last model prior to its training in last step may be crucial for efficiency of algorithm.\\
    There are several possible ways to set weights of last model:
    \begin{itemize}
        \item \textbf{Classic} ~-- Use default (untrained) initialization. This approach may cause corresponding convex coefficient to approach zero (as other models produce much better results); which in turn causes gradients of the last model's parameters to be excessively small and effectively disables its training.
        \item \textbf{Pretrained} ~-- fully train the last model prior to the last step. This, on the other hand, may cause the last model to not be trained sufficiently, as star model may start close to a local minimum (model average ensemble).
        \item \textbf{Warm-up} ~-- train the last model for several epoches prior to the last step. On one hand, in this case the last model produces adequate results on its own; on the other hand star model will not be stuck in local minima and may train sufficiently well.
    \end{itemize}
    This variants may also be applied to snapshot modification of star algorithm. However, fully training the last model in addition to snapshot models highly increases computational expenses, rendering snapshot technique ineffective. Therefore, to preserve training budget, the last snapshot is used for the pretrained variant.\\
